Probing the Dispersion and Rotation Measure Contributions from Supernova Remnants in Fast Radio Burst Source Environments with 1D SNR Simulation

Fast radio bursts (FRBs) provide a sensitive probe of ionized baryons through their dispersion measure (DM). In addition to slowly evolving cosmological terms, at least two repeaters now show clear secular DM-decrease episodes: FRB~20190520B and FRB~20121102 , supporting a dense, dynamically evolving local environment. We adopt a \emph{forward-modeling} approach and use time-dependent 1D SNR simulations for a young magnetar embedded in SN ejecta, combining single-star and binary-stripped progenitors with HD+NEI calculations to follow shock structure, ionization, and electron density. The shocked region contributes only limited DM ($\lesssim10\,{\rm pc\,cm^{-3}}$), while the dominant time-varying component is the unshocked ejecta, whose early behavior follows ${\rm DM}\propto t^{-\alpha}$ with $\alpha\simeq1.8$--$1.9$. Although shocked-region DM is small, shock-amplified magnetic fields can still generate substantial RM; in our shock-only RM framework, only the $11\,M_\odot$ SS model reproduces the FRB~20121102 RM evolution. Binary-stripped progenitors generally yield smaller DM than single-star models at fixed $M_{\rm ZAMS}$, with composition-dependent mean molecular weights introducing non-monotonic mass trends. Matching the observed ${\rm dDM}/{\rm d}t$ of FRB~20190520B (and the late-stage slope of FRB~20121102), we infer local SNR DM contributions of tens to hundreds ${\rm pc\,cm^{-3}}$. We also find GHz escape is allowed in most models, with $\tau_{\rm ff}=1$ typically reached by $t_{\rm esc}\lesssim70$ yr; for weakly ionized ejecta, the source can be nearly transparent from very early times. These results support a young CCSN/SNR origin for a substantial fraction of ${\rm DM}_{\rm source}$ and highlight that physically consistent local-environment modeling is essential for robust FRB cosmological DM inferences.

==> Bibtex.tex <==
\begin{thebibliography}{}
\expandafter\ifx\csname natexlab\endcsname\relax\def\natexlab#1{#1}\fi
\providecommand{\url}[1]{\href{#1}{#1}}
\providecommand{\dodoi}[1]{doi:~\href{http://doi.org/#1}{\nolinkurl{#1}}}
\providecommand{\doeprint}[1]{\href{http://ascl.net/#1}{\nolinkurl{http://ascl.net/#1}}}
\providecommand{\doarXiv}[1]{\href{https://arxiv.org/abs/#1}{\nolinkurl{https://arxiv.org/abs/#1}}}
% 参考文献部分
\bibitem[Cen(2012)]{Cen2012ApJ...753...17C} Cen, R.\ 2012, \apj, 753, 17. doi:10.1088/0004-637X/753/1/17

\bibitem[Cen \& Ostriker(1999)]{CO1999ApJ...514....1C} Cen, R. \& Ostriker, J.~P.\ 1999, \apj, 514, 1. doi:10.1086/306949

\bibitem[CHIME/FRB Collaboration et al.(2021)]{2021ApJS..257...59C} CHIME/FRB Collaboration, Amiri, M., Andersen, B.~C., et al.\ 2021, \apjs, 257, 59. doi:10.3847/1538-4365/ac33ab

\bibitem[Chime/FRB Collaboration et al.(2023)]{2023ApJS..264...53C} Chime/Frb Collaboration, Amiri, M., Andersen, B.~C., et al.\ 2023, \apjs, 264, 53. doi:10.3847/1538-4365/acb54c


\bibitem[Danforth \& Shull(2005)]{DS2005ApJ...624..555D} Danforth, C.~W. \& Shull, J.~M.\ 2005, \apj, 624, 555. doi:10.1086/429285

\bibitem[Danforth \& Shull(2008)]{DS2008ApJ...679..194D} Danforth, C.~W. \& Shull, J.~M.\ 2008, \apj, 679, 194. doi:10.1086/587127

\bibitem[Dav{\'e} et al.(2001)]{Dave2001ApJ...552..473D} Dav{\'e}, R., Cen, R., Ostriker, J.~P., et al.\ 2001, \apj, 552, 473. doi:10.1086/320548

\bibitem[Fukushima et al.(2023)]{Fukushima2023MNRAS.525.3760F} Fukushima, K., Nagamine, K., \& Shimizu, I.\ 2023, \mnras, 525, 3760. doi:10.1093/mnras/stad2526

\bibitem[Khrykin et al.(2024)]{Khrykin2024arXiv240200505K} Khrykin, I.~S., Ata, M., Lee, K.-G., et al.\ 2024, arXiv:2402.00505. doi:10.48550/arXiv.2402.00505

\bibitem[Khrykin et al.(2024)]{Khrykin2024MNRAS.529..537K} Khrykin, I.~S., Sorini, D., Lee, K.-G., et al.\ 2024, \mnras, 529, 537. doi:10.1093/mnras/stae525

\bibitem[Lee et al.(2022)]{Lee2022} Lee, K.-G., Ata, M., Khrykin, I.~S., et al.\ 2022, \apj, 928, 9. doi:10.3847/1538-4357/ac4f62

\bibitem[Lee et al.(2023)]{Lee2023} Lee, K.-G., Khrykin, I.~S., Simha, S., et al.\ 2023, \apjl, 954, L7. doi:10.3847/2041-8213/acefb5

\bibitem[Lorimer et al.(2007)]{Lorimer2007} Lorimer, D.~R., Bailes, M., McLaughlin, M.~A., et al.\ 2007, Science, 318, 777. doi:10.1126/science.1147532

\bibitem[Macquart et al.(2020)]{Macquart2020Nature} Macquart, J.-P., Prochaska, J.~X., McQuinn, M., et al.\ 2020, \nat, 581, 391. doi:10.1038/s41586-020-2300-2

\bibitem[Nicastro et al.(2005a)]{Nicastro2005a} Nicastro, F., Mathur, S., Elvis, M., et al.\ 2005a, \nat, 433, 495. doi:10.1038/nature03245

\bibitem[Nicastro et al.(2005b)]{Nicastro2005b} Nicastro, F., Mathur, S., Elvis, M., et al.\ 2005b, \apj, 629, 700. doi:10.1086/431270

\bibitem[Oku et al.(2022)]{Oku2022} Oku, Y., Tomida, K., Nagamine, K., et al.\ 2022, \apjs, 262, 9. doi:10.3847/1538-4365/ac77ff

\bibitem[Prochaska et al.(2011)]{Prochaska2011ApJ...740...91P} Prochaska, J.~X., Weiner, B., Chen, H.-W., et al.\ 2011, \apj, 740, 91. doi:10.1088/0004-637X/740/2/91

\bibitem[Salucci \& Persic(1999)]{Salucci1999MNRAS.309..923S} Salucci, P. \& Persic, M.\ 1999, \mnras, 309, 923. doi:10.1046/j.1365-8711.1999.02913.x

\bibitem[Reiprich \& B{\"o}hringer(2002)]{Reiprich2002ApJ...567..716R} Reiprich, T.~H. \& B{\"o}hringer, H.\ 2002, \apj, 567, 716. doi:10.1086/338753

\bibitem[Rybicki \& Lightman(1979)]{RL1979rpa..book.....R} Rybicki, G.~B. \& Lightman, A.~P.\ 1979, A Wiley-Interscience Publication, New York: Wiley, 1979

\bibitem[Richter et al.(2006)]{Richter2006} Richter, P., Savage, B.~D., Sembach, K.~R., et al.\ 2006, \aap, 445, 827. doi:10.1051/0004-6361:20053636

\bibitem[Richter et al.(2004)]{Richter2004} Richter, P., Savage, B.~D., Tripp, T.~M., et al.\ 2004, \apjs, 153, 165. doi:10.1086/421297

\bibitem[Simha et al.(2023)]{Simha2023ApJ...954...71S} Simha, S., Lee, K.-G., Prochaska, J.~X., et al.\ 2023, \apj, 954, 71. doi:10.3847/1538-4357/ace324

\bibitem[Shimizu et al.(2019)]{Shimizu2019MNRAS.484.2632S} Shimizu, I., Todoroki, K., Yajima, H., et al.\ 2019, \mnras, 484, 2632. doi:10.1093/mnras/stz098

\bibitem[Sorini et al.(2022)]{Sorini2022MNRAS.516..883S} Sorini, D., Dav{\'e}, R., Cui, W., et al.\ 2022, \mnras, 516, 883. doi:10.1093/mnras/stac2214

\bibitem[So{\l}tan(2006)]{Sotan2006A&A...460...59S} So{\l}tan, A.~M.\ 2006, \aap, 460, 59. doi:10.1051/0004-6361:20065431

\bibitem[Thornton et al.(2013)]{Thornton2013} Thornton, D., Stappers, B., Bailes, M., et al.\ 2013, Science, 341, 53. doi:10.1126/science.1236789

\bibitem[Tilton et al.(2012)]{Tilton2012ApJ...759..112T} Tilton, E.~M., Danforth, C.~W., Shull, J.~M., et al.\ 2012, \apj, 759, 112. doi:10.1088/0004-637X/759/2/112

\bibitem[Tripp et al.(2006)]{Tripp2006ASPC..348..341T} Tripp, T.~M., Bowen, D.~V., Sembach, K.~R., et al.\ 2006, Astrophysics in the Far Ultraviolet: Five Years of Discovery with FUSE, 348, 341

\bibitem[Wang \& Wei(2023)]{Wang2023ApJ...944...50W} Wang, B. \& Wei, J.-J.\ 2023, \apj, 944, 50. doi:10.3847/1538-4357/acb2c8

\bibitem[Yang et al.(2022)]{Yang2022ApJ...940L..29Y} Yang, K.~B., Wu, Q., \& Wang, F.~Y.\ 2022, \apjl, 940, L29. doi:10.3847/2041-8213/aca145

\bibitem[Yao et al.(2012)]{Yao2012ApJ...746..166Y} Yao, Y., Shull, J.~M., Wang, Q.~D., et al.\ 2012, \apj, 746, 166. doi:10.1088/0004-637X/746/2/166

\bibitem[Yoshikawa et al.(2001)]{Yoshikawa2001ApJ...558..520Y} Yoshikawa, K., Taruya, A., Jing, Y.~P., et al.\ 2001, \apj, 558, 520. doi:10.1086/322445

\bibitem[Zwaan et al.(2003)]{Zwaan2003AJ....125.2842Z} Zwaan, M.~A., Staveley-Smith, L., Koribalski, B.~S., et al.\ 2003, \aj, 125, 2842. doi:10.1086/374944

\bibitem[Persic \& Salucci(1992)]{1992MNRAS.258P..14P} Persic, M. \& Salucci, P.\ 1992, \mnras, 258, 14P. doi:10.1093/mnras/258.1.14P

\bibitem[Bristow \& Phillipps(1994)]{BP1994} Bristow, P.~D. \& Phillipps, S.\ 1994, \mnras, 267, 13. doi:10.1093/mnras/267.1.13

\bibitem[Fukugita et al.(1998)]{1998ApJ...503..518F} Fukugita, M., Hogan, C.~J., \& Peebles, P.~J.~E.\ 1998, \apj, 503, 518. doi:10.1086/306025

\end{thebibliography}{}

==> Response_to_Referee <==
We thank the referee and the editor for their careful reading of the manuscript and for their constructive comments. We have revised the manuscript accordingly and addressed all points raised. A detailed, point-by-point response is provided below.

Reviewer #1:

The manuscript is well written and I have only minor remarks

ll. 21-22
>>combining single-star and binary-stripped progenitors with HD+NEI calculations
Define all abbreviations (HD, NEI) on first use in the abstract

Response:
We thank the referee for pointing this out. We have now defined the abbreviations in the abstract as “hydrodynamic (HD) and non-equilibrium ionization (NEI)”  in Line 22

ll. 74-76
>>On timescales of ∼years, all components except DMsource are expected to be negligible

'changes in' were lost.

Response:
We thank the referee for pointing this out. We have revised the sentence in Line 77 to read “temporal variations in all components except DM_source are expected to be negligible,”.

ll. 210-213
>>Here DMdiff traces large-scale structure along the line of sight and is the component that can be robustly estimated from cosmological simulations or empirical DM- z relations.

'Robustly' is a bit of exaggeration.

Response:
We thank the referee for this suggestion. We have replaced “robustly estimated” with “reasonably well estimated” to avoid overstatement in Lines 226-227.

ll. 507-508
>>and both the wind and ISM temperatures are set to T = 10^4 K.
Why the wind temperature was set at this value and how did it affect the calculations?

Response:
We thank the referee for this question. The choice of T = 10^4 K is intended to represent a warm photoionized ambient medium and to avoid introducing an artificially cold initial pressure floor. This clarification has been added to the manuscript (Lines 525–527). 

ll. 576-577
>>In our setup, RCSM,max = 39.9 Mpc is set by the initial conditions
Why this value is so large, crawling not only into the HG territory but into the IGM proper? What are the justifications for this limit and why natural Rmax~100 pc wouldn't work?

Response:
We apologize for making confusion. This was a typographical error in the manuscript. The correct value is R_{\rm CSM,max} = 39.9 pc, not Mpc.  This scale is consistent with the typical size of the circumstellar medium in our model. We have corrected this in the revised manuscript (Lines 596-600).


ll. 639
>> which will be compared with observatMatchingionally

A misprint

Response:
The typo has been corrected to “observationally inferred” in the revised manuscript (Lines 662-663).

ll. 659
>> RM is then obtained by integrating neB∥ along the line
The authors should explicitly add the coefficient, that links B|| to (or B?). Also, do the authors imply that the field is completely ordered?
This point should be clarified.

Response:
  We thank the referee for this important comment. We have now explicitly included the coefficient in the RM calculation, such that “RM = 0.81 ∫ n_e B_\parallel dl, with n_e in cm^{-3}, B_\parallel in \mu G, and dl in pc”.
We have also clarified that our calculation adopts an effective line-of-sight magnetic field and does not explicitly model small-scale tangling or reversals of magnetic fields. This has been stated in the revised manuscript (Lines 671–675).


ll. 1276-1280.
>>As a result, potentially important CR- related processes-including escaping CR particles and CR-driven magnetic-field amplification (e.g., streaming instabilities and Bell-type instabilities)-are absent.

Could these processes include additional ionization, caused by the escaping CRs?

Response: 
  We thank the referee for this insightful question. We have added a clarification noting that escaping cosmic rays could, in principle, contribute additional ionization and enhance the electron density. However, these effects are not included in the present model, and their quantitative impact remains uncertain. This discussion has been added to the manuscript (Lines 1326–1334).

ll. 1373-1376
>>A common conclusion from both FRB 20190520B and FRB 121102 is that the inferred local SNR contribution falls in the tens-to-hundreds pc cm−3 range.

There could be a very important corollary, given that the non-repeaters are most likely older sources. What are the typical DM values, predicted for them from the simulations? Could it mean, that the DMsource term could be safely ignored for them?


Response:
  We thank the referee for this insightful comment. If non-repeating FRBs are associated with older source populations, our results are consistent with the expectation that their local SNR contributions to DM would be significantly reduced at late times, potentially becoming subdominant compared to other components. In this regime, the DM_source term may become subdominant compared to other contributions.

However, we note that the age distribution and physical origins of non-repeating FRBs remain uncertain. While the source contribution is likely reduced at late times, it may not be universally negligible. We have added a discussion of this point in the revised manuscript (Lines 1449–1461).

Additional Response:

We have added a new citation to Margalit et al. (2018) in Line 59..


Regarding FRB~20220529A:

In the revised manuscript, we have incorporated the latest observational update on FRB~20220529A and treated it as an additional benchmark source alongside FRB~20190520B and FRB~20121102. Specifically, we added the recent monitoring result showing a secular DM decline of dDM/dt = -0.881 pc cm^{-3} yr^{-1} (see Abstract, lines 17–19, 29-31; Introduction, lines 127–136).

We then extended our SNR slope-matching analysis to FRB~20220529A and quantified the inferred occurrence time and DM derivatives in local SNR DM contribution in the same framework used for the other repeaters  (see Section 5.2.2 and 5.2.3, Lines 1098–1118, 1133-1164, 1407-1416, 1429-1449). 

In the fiducial ionization configuration, the observed slope of FRB~20220529A implies t_occur ~ 67 yr (11 $M_\odot$ SS), 18 yr (11 $M_\odot$ BS), 74 yr (30 $M_\odot$ SS), and 61 yr (30 $M_\odot$ BS), see Table 6. The corresponding inferred local SNR contributions are systematically smaller than those for FRB~20190520B and FRB~20121102, falling in the range DM_{SNR} ~ 12.4--36.1 pc cm^{-3} (Table 2).  We believe this addition improves the completeness and timeliness of the revised manuscript and further demonstrates that our framework can accommodate the newly reported secular DM evolution of FRB~20220529A in a self-consistent way.


----------------------------------------------------------------------
Data Editor's Review:

One of our expert data editors has reviewed your initial manuscript submission and has the following suggestion(s) to help improve the data, software citation and/or overall content. Please treat this as you would a reviewer's comments and respond accordingly in your report to the science editor. Questions can be sent directly to the data editors at data-editors@aas.org.

You mention in your Data Availability statement that "The data presented in this paper is available to the research community upon request to the authors." However, we strongly recommend that vital data in support of this work is either deposited with the article as data behind a figure [1] or deposited into a DOI-issuing repository such as Zenodo [2] with the dataset DOI added to the text using the AASTeX \dataset[]{} command [3]. This deposit is important for the preservation of your data and substantially reduces the barrier to the reuse of these results. Please ensure that the available data is described in your paper.

[1] https://journals.aas.org/data-guide/#data_behind_figures
[2] https://github.com/AASJournals/Tutorials/tree/master/Repositories
[3] https://journals.aas.org/aastexguide/#datasets


Response:
We thank the data editor for the helpful suggestion.

The SNR simulations in this work are based on a customized, non-public code, and therefore the full simulation pipeline cannot be made publicly available at this stage. However, we agree on the importance of data accessibility and reproducibility.

We note that part of our analysis framework is publicly available through our ARCOS codebase (https://github.com/zhaojosephzhang/ARCOS), which is primarily developed for FRB cosmology and simulation-based analysis. We plan to incorporate the SNR source analysis components presented in this work into this codebase in future releases.

In the revised manuscript, we have clarified the Data Availability statement and added a more detailed description of the data products used in this work. The derived data supporting the figures and main results (e.g., DM and RM evolution profiles) can be made available upon reasonable request.

We will also consider depositing selected data products (e.g., data behind figures) in a public repository such as Zenodo in future work.


We thank the referee and the editor again for their constructive comments. We hope that the revisions have adequately addressed all concerns and improved the clarity of the manuscript.



